Large-scale Multiview 3D Hand Pose Dataset

Accurate hand pose estimation at joint level has several uses on human-robot interaction, user interfacing and virtual reality applications. Yet, it currently is not a solved problem. The novel deep learning techniques could make a great improvement on this matter but they need a huge amount of annotated data. The hand pose datasets released so far present some issues that make them impossible to use on deep learning methods such as the few number of samples, high-level abstraction annotations or samples consisting in depth maps. In this work, we introduce a multiview hand pose dataset in which we provide color images of hands and different kind of annotations for each, i.e the bounding box and the 2D and 3D location on the joints in the hand. Besides, we introduce a simple yet accurate deep learning architecture for real-time robust 2D hand pose estimation.

==> future_work.tex <==
\section{Future Work}
\label{sec:future_work}

Following on this work we plan to design a new architecture for robust 3D hand pose estimation in which the system will provide not only x and y coordinates in the image plane but x, y and z, and the normal of the palm on real world coordinates.
